Right Makes Might: Aligning Verified Hidden States Empowers RL Reasoning

Reinforcement Learning from Verifiable Rewards (RLVR) has become the dominant approach for improving mathematical reasoning in large language models, yet current methods reduce each correct rollout to a single reward bit, ignoring the geometric structure shared among their hidden states. Investigating this structure, we find that at the anchor token (the position immediately before the answer marker), correct rollouts converge naturally because they must produce the same answer (cosine similarity ~0.84), yet each retains residual variance from its unique reasoning path. Encouraging full alignment at this point pushes the model to extract a unified "correct decision" representation, reducing sensitivity to which reasoning path was taken. Based on this observation, we propose Hidden-Align, an auxiliary loss function that aligns the last-layer hidden states of correct rollouts at the anchor token during RL training, with zero overhead in both training and inference. On eight mathematical reasoning benchmarks, Hidden-Align improves average pass@1 over the DAPO baseline by 3.8, 6.2, and 5.4 percentage points on Qwen3-1.7B, 4B, and 14B respectively, with consistent pass@k gains across all three scales, supported by ablations on loss type, anchor position, layer depth, and loss weight.

==> sections_main/preamble.tex <==
% Additional packages (avoid duplicating what acl_latex.tex already loads)
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage[noend]{algpseudocode}
\usepackage{adjustbox}
\usepackage{colortbl}
\usepackage{xspace}
\usepackage{subcaption}
\usepackage{pifont}
\usepackage{float}

% --- colors
\definecolor{demphcolor}{RGB}{144, 144, 144}
\definecolor{mygray}{gray}{0.4}
\definecolor{my_green}{RGB}{51,102,0}
\definecolor{my_red}{RGB}{204, 0, 0}
\definecolor{suffblue}{RGB}{74,144,217}
\definecolor{insufforange}{RGB}{232,115,74}

% --- commands
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\impro}[1]{{\hspace{0.05cm}{\color[HTML]{32CB00}\textbf{(+#1)}}}}
\newcommand{\degra}[1]{{\hspace{0.05cm}{\textcolor{red}{\textbf{(-#1)}}}}}
\newcommand{\demph}[1]{\textcolor{demphcolor}{#1}}
\newcommand{\cmark}{\textcolor{my_green}{\ding{51}}}
\newcommand{\xmark}{\textcolor{my_red}{\ding{55}}}

\newcommand{\modelname}{Hidden-Align\xspace}


==> tables/baselines.tex <==

\begin{table*}[]
\small
\caption{Comparison with baseline methods across various evaluation metrics. Our method achieves the best performance on most metrics, while \modeldpo demonstrates performance comparable to \modelname. Bold text indicates the best results, and underlined text denotes the second-best.
}
\label{tab:base}
\begin{tabular}{l|cccc|cccc|c|c}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{CapsBench}    & \multicolumn{4}{c|}{CompreCap}     &  \multicolumn{1}{c|}{Amber}    & \multirow{2}{*}{Capture}  \\ \cmidrule{2-10}
       
     & Acc. & Color & Shape & Rel. Pos. & Obj.    & Pix.   & Rel.    & Attr. & Over.  \\ \midrule
     
LaCLIP~(\citeauthor{laclip})       & 22.65  & 21.65    & 9.09  &  11.11 & 48.02   & 42.59    & 1.73   & 2.29    &    43.8     &      39.56          \\ 
CapsFusion~(\citeauthor{capsfusion})     & 35.04  & 38.14  &12.12   & 25.46  & 61.67 & 52.63      & 2.32   & 2.59   &  44.5   &     56.03           \\ 
Self-Loop~(\citeauthor{capture})     & 29.63  & 29.55  &  9.09   & 17.13   & 65.77    & 51.54  & 2.30    & 2.53    & 49.5           &     56.61      

\\ 

VeCLIP~(\citeauthor{veclip}) &25.19  & 27.84   &   11.11     & 13.43   & 49.60 &  42.25   &2.50  &     1.77       &     41.0    & 38.13 \\ 

ShareGPT4V~(\citeauthor{sharegpt4v}) &50.46  & 62.13   &   38.78   & 49.34  & 67.47 &  62.00   &2.83  &     2.81       &     56.2   & 59.80 \\ 
% Patch Matters & \\
\midrule
    \modeldpo (Ours)    & \underline{55.32} & \underline{66.67} & \underline{50.29} & \underline{55.09} &    \underline{74.80}   & \textbf{63.35} & \underline{2.84} & \textbf{2.84}  & \underline{60.6} & \underline{65.52}   \\ 

\modelname (Ours)&    \textbf{59.02} & \textbf{67.14} & \textbf{53.68} & \textbf{59.51}  & \textbf{75.04} & \underline{63.04} & \textbf{2.85} & \underline{2.82} &        \textbf{62.2}    &  \textbf{65.98}            \\ \bottomrule[1.5pt]
\end{tabular}
\end{table*}

% \begin{table*}[]
% \small
% \caption{Comparison with baseline methods across various evaluation metrics. Our method achieves the best performance on most metrics, while \modeldpo demonstrates performance comparable to \modelname. Bold text indicates the best results, and underlined text denotes the second-best.
% }
% \label{tab:base}
% \begin{tabular}{l|c|c|cccc|cccc}
% \toprule[1.5pt]
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{Capture} & Amber & \multicolumn{4}{c|}{CapsBench}    & \multicolumn{4}{c}{CompreCap}    \\ \cmidrule{4-11}
       
%      &  & Over. & Acc. & Color & Shape & Rel. Pos. & Obj.    & Pix.   & Rel.    & Attr.  \\ \midrule
     
% LaCLIP~(\citeauthor{laclip})       & 39.56 & 43.8 & 22.65  & 21.65    & 9.09  &  11.11 & 48.02   & 42.59    & 1.73   & 2.29  \\ 
% CapsFusion~(\citeauthor{capsfusion})     & 56.03 & 44.5 & 35.04  & 38.14  &12.12   & 25.46  & 61.67 & 52.63      & 2.32   & 2.59  \\ 
% Self-Loop~(\citeauthor{capture})     & 56.61 & 49.5 & 29.63  & 29.55  &  9.09   & 17.13   & 65.77    & 51.54  & 2.30    & 2.53  \\ 
% VeCLIP~(\citeauthor{veclip}) & 38.13 & 41.0 & 25.19  & 27.84   &   11.11     & 13.43   & 49.60 &  42.25   &2.50  &     1.77  \\ 
% ShareGPT4V~(\citeauthor{sharegpt4v}) & 59.80 & 56.2 & 50.46  & 62.13   &   38.78   & 49.34  & 67.47 &  62.00   &2.83  &     2.81  \\ 
% \midrule
% \modeldpo (Ours)    & \underline{65.52} & \underline{60.6} & \underline{55.32} & \underline{66.67} & \underline{50.29} & \underline{55.09} & \underline{74.80}   & \textbf{63.35} & \underline{2.84} & \textbf{2.84}  \\ 
% \modelname (Ours)& \textbf{65.98} & \textbf{62.2} & \textbf{59.02} & \textbf{67.14} & \textbf{53.68} & \textbf{59.51}  & \textbf{75.04} & \underline{63.04} & \textbf{2.85} & \underline{2.82} \\ 
% \bottomrule[1.5pt]
% \end{tabular}
% \end{table*}



==> tables/clair.tex <==
\begin{table}[t] 
\small
\begin{center}
\caption{Performance on CLAIR metric.}
\label{tab:clair}
\begin{tabular}{l|c}
\toprule[1.5pt]
Methods & CLAIR  \\ 
\midrule
LaCLIP & 0.749 \\
CapsFusion	&0.795 \\
RICO-Flash	&0.839 \\
RICO	&0.864 \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table}


==> tables/compare.tex <==
\begin{table}[t] 
\small
\begin{center}
\caption{Performance of different comparison methods.}
\label{tab:comparison}
\begin{tabular}{l|c}
\toprule[1.5pt]
Methods & Capsbench Acc.  \\ 
\midrule
Original Qwen2-VL & 43.55 \\
+ Image-text comparison	&49.50 \\
+ Image-image comparison	&54.08 \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table}


==> tables/consistency.tex <==
\begin{table}[t] 
\small
\begin{center}
\caption{Evaluations using different models.}
\label{tab:eval_diff}
\begin{tabular}{l|c}
\toprule[1.5pt]
Model Used for Evaluation &	CapsBench Acc.  \\ 
\midrule
GPT-4o & 59.0 \\
GPT-4v	&58.7 \\
Gemini 2.5pro	&59.2 \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table}


==> tables/gemini.tex <==
\begin{table}[t] 
\small
\begin{center}
\caption{Results on CapsBench, evaluated by Gemini 2.5 Pro.}
\label{tab:eval_gem}
\begin{tabular}{l|c}
\toprule[1.5pt]
Models	& CapsBench \\
\midrule
LaCLIP	&23.4 \\
CapsFusion	&34.7\\
Self-Loop	&30.4\\
VeCLIP	&23.5\\
ShareGPT4V	&50.6\\
RICO-Flash	&54.3\\
RICO	& 59.2\\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table}


==> tables/human.tex <==
\begin{table}[t] 
\small
\begin{center}
\tabcolsep=0.2cm
\caption{Recaptioning results by humans and models based on the initial caption. In our \modelname method, a single iteration of refinement is performed.
}
	\label{tab:human}
	\begin{tabular}{l|cccc}
		\toprule[1.5pt]
		 \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{CapsBench (Subset)}   \\  
         \cmidrule{2-5}
        & Acc. & Color  & Rel. Pos. & Shape\\
        \midrule
        Original & 43.55 & 44.30 & 39.45 & 20.41 \\
        + GPT-4o Edit & 49.50 &53.02 &44.04 &24.49   \\
        + Human Edit & 50.96 & 51.30 & 47.82 & 27.01  \\
        + \modelname Edit & \textbf{54.08} & \textbf{65.47} & \textbf{34.04} & \textbf{49.51} \\
	\bottomrule[1.5pt]
	\end{tabular}

\end{center}

\end{table}

==> tables/human_inst.tex <==
\begin{table}[ht!]
\caption{Instructions provided to human annotators in the caption editing experiment.
}

\begin{tcolorbox}

{\normalsize \textbf{==  ~\textsc{Instruction to annotators}~ ==}}

\tcblower


We are working on an image captioning task. The following caption was generated by an AI model. Please help refine this caption by correcting any errors or ambiguities based on the image, and feel free to add any important details that are missing from the original caption.


\end{tcolorbox}

\label{tab:human_ins}
\end{table}

==> tables/init_all.tex <==
\begin{table*}[]
\small
\caption{Detailed performance of \modelname across different initial captioning models.}
\label{tab:app_init}
\tabcolsep=0.03cm
\begin{tabular}{l|llll|llll}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{CapsBench}    & \multicolumn{4}{c}{CompreCap}      \\ \cmidrule{2-9}

 & Acc. & Color & Shape & Rel. Pos. & Obj.    & Pix.   & Rel.    & Attr.  \\ \midrule[1pt]
 
% qwen                                      & \multicolumn{1}{l|}{42.02\%/59.02\% (+ 17\%)}    & \multicolumn{1}{l|}{48.11/67.14} & 32,41/59.51       & \multicolumn{1}{l|}{-}                      & \multicolumn{1}{l|}{-}                      & \multicolumn{1}{l|}{-}               & -                \\ \hline
% cogvlm                                    & \multicolumn{1}{l|}{45.1\%/57.51\% (+12.41\%)}   & \multicolumn{1}{l|}{47.77/63.67} & 39.81/48.76       & \multicolumn{1}{l|}{68.54\%/75.37\%(+6.83)} & \multicolumn{1}{l|}{59.21\%/61.65\%(+2.44)} & \multicolumn{1}{l|}{2.57/2.78(0.21)} & 2.61/2.75(+0.14) \\ \hline
% gpt4o                                     & \multicolumn{1}{l|}{43.52\%/54.58\% (+11.06\%)}  & \multicolumn{1}{l|}{48.11/65.85} & 30.09/53.08       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                &                  \\ \hline
% gemini                                    & \multicolumn{1}{l|}{49.71\%/57.72\% (+ 8.01\%)}  & \multicolumn{1}{l|}{51.2/65.7}   & 36.57/50.48       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                &                  \\ \hline
% blip3                                     & \multicolumn{1}{l|}{37.03\%/56.21\% (+ 19.18\%)} & \multicolumn{1}{l|}{40.55/66.2}  & 29.63/55.61       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                &                  \\ \hline
% LLaVA 1.5                                     & \multicolumn{1}{l|}{29.51\%/53.13\% (+ 23.62\%)} & \multicolumn{1}{l|}{27.84/61.07} & 18.06/48.1        & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                &                  \\ \hline


Qwen2-VL (\citeauthor{qwen2vl}) & 42.02 & 48.11 & 27.27 & 32.41 & 69.82  & 60.02  & 2.66 & 2.81 \\
Qwen2-VL + \modelname & 59.02$_\impro{17.00}$ & 67.14$_\impro{19.03}$ & 53.68$_\impro{26.41}$ & 59.51$_\impro{27.10}$ & 75.04$_\impro{5.22}$ & 63.04$_\impro{3.02}$ & 2.85$_\impro{0.19}$ & 2.82$_\impro{0.01}$ \\
\midrule

CogVLM 2 (\citeauthor{hong2024cogvlm2visuallanguagemodels}) & 45.10 & 47.77 & 28.23 & 39.81 & 68.54 & 59.21 & 2.57 & 2.61 \\
CogVLM 2 + \modelname & 57.51$_\impro{12.41}$ & 63.67$_\impro{15.90}$ & 35.46$_\impro{7.23}$ & 48.76$_\impro{8.95}$ & 75.37$_\impro{6.83}$ & 61.65$_\impro{2.44}$ & 2.78$_\impro{0.21}$ & 2.75$_\impro{0.14}$ \\
\midrule

GPT-4o (\citeauthor{openai2024gpt4ocard}) & 49.63 & 54.64 & 28.28 & 48.15 & 70.93 & 60.09 & 2.67 & 2.77 \\
GPT-4o + \modelname & 57.68$_\impro{8.05}$ & 63.24$_\impro{8.60}$ & 44.57$_\impro{16.29}$ & 59.47$_\impro{11.32}$ & 74.47$_\impro{3.54}$ & 62.11$_\impro{2.02}$ & 2.76$_\impro{0.09}$ & 2.81$_\impro{0.04}$ \\
\midrule

Gemini 1.5 Pro (\citeauthor{geminiteam2024gemini15unlockingmultimodal}) & 49.71 & 51.20 & 23.23 & 36.57 & 71.77 & 60.28 & 2.89 & 2.71 \\
Gemini 1.5 Pro + \modelname & 57.72$_\impro{8.01}$ & 65.70$_\impro{14.50}$ & 37.50$_\impro{14.27}$ & 50.48$_\impro{13.91}$ & 75.77$_\impro{4.00}$ & 61.97$_\impro{1.69}$ & 2.85$_\impro{-0.04}$ & 2.83$_\impro{0.12}$ \\
\midrule

BLIP-3~(\citeauthor{xue2024xgenmmblip3familyopen}) & 37.03 & 40.55 & 19.19 & 29.63 & 67.85 & 56.99 & 2.61 & 2.50 \\
BLIP-3 + \modelname & 56.21$_\impro{19.18}$ & 66.20$_\impro{25.65}$ & 37.76$_\impro{18.57}$ & 55.61$_\impro{25.98}$ & 74.31$_\impro{6.46}$ & 61.47$_\impro{4.48}$ & 2.79$_\impro{0.18}$ & 2.75$_\impro{0.25}$ \\
\midrule

LLaVA 1.5 (\citeauthor{llava}) & 29.51 & 27.84 & 9.09 & 18.06 & 57.14 & 44.48 & 2.02 & 2.38 \\
LLaVA 1.5 + \modelname & 53.13$_\impro{23.62}$ & 61.07$_\impro{33.23}$ & 36.84$_\impro{27.75}$ & 48.10$_\impro{30.04}$ & 76.38$_\impro{19.24}$ & 61.49$_\impro{17.01}$ & 2.82$_\impro{0.80}$ & 2.82$_\impro{0.44}$ \\



\bottomrule[1.5pt]
\end{tabular}
\end{table*}


==> tables/init_prompt_templa.tex <==
\begin{table*}[ht!]
\caption{Different prompts used to generate initial captions.
}

\begin{tcolorbox}

{\normalsize \textbf{============  ~\textsc{Different prompts to generate initial captions}~ ============}}

\tcblower


Prompt \#1: Describe this image in detail. Your answer should be concise and informative.
~\\

Prompt \#2: Describe the image with rich and detailed observations. You may pay attention to the dimensions of overall, main subject, background, movement of main subject, style, camera movement and so on.
~\\

Prompt \#3: Give this image a detailed caption.



\end{tcolorbox}

\label{tab:initial_prompt}
\end{table*}

==> tables/initial.tex <==
% \begin{table}[t] 
% \small
% \begin{center}
% \tabcolsep=0.15cm
% \caption{Generality of \modelname across different initial recaptioning models and prompts.
% }
% \vspace{-1mm}
% 	\label{tab:rob}
% 	\begin{tabular}{l|c|c}
% 		\toprule[1.5pt]
% 		 Model  &
%          CapsBench (Acc) & CompreCap (Uni.)   \\        \midrule
%         GPT-4o & 49.63 / 57.68$_\impro{}$ & 58.58 / 60.36
%           \\
%         Gemini 1.5 Pro                                   & 49.71 / 57.72\impromath{8.01} & 60.07 / 61.52\\
%         BLIP-3~\cite{}                                     & 37.03 / 56.21\impromath{19.18} & 55.38 / 60.18\impromath{}\\
%         % LLaVA 1.5                                     & 29.51 /53.13\impromath{23.62} \\ 
%         CogVLM 2 & 45.10 / 57.51 & 55.97 / 60.33 \\ \midrule

%          Qwen2-VL (Prompt 1)                                    & 42.02 / 59.02$_\impro{17.00}$ & 55.90 / 61.36\\
%           Qwen2-VL (Prompt 2) & 45.97 / 57.64$_\impro{}$ & 57.21 / 60.60  \\
%         Qwen2-VL (Prompt 3)   & 41.85 / 54.85\impromath{} & 56.94 / 60.90 \\
% 		\bottomrule[1.5pt]
% 	\end{tabular}

% \end{center}

% \end{table}

\begin{table}[t] 
\small
\begin{center}
\tabcolsep=0.08cm
\caption{Generality of \modelname across different initial recaptioning models and prompts. For CapsBench, we report overall accuracy, and for CompreCap, we use the unified metric for evaluation.}
\vspace{-1mm}
\label{tab:rob}
\begin{tabular}{l|c|c}
\toprule[1.5pt]
Model & CapsBench & CompreCap \\ 
\midrule
GPT-4o & 49.6 / 57.7$_\impro{8.1}$ & 58.6 / 60.4$_\impro{1.8}$ \\
Gemini 1.5 Pro & 49.7 / 57.7$_\impro{8.0}$ & 60.1 / 61.5$_\impro{1.4}$ \\
BLIP-3 & 37.0 / 56.2$_\impro{19.2}$ & 55.4 / 60.2$_\impro{4.8}$ \\
CogVLM 2 & 45.1 / 57.5$_\impro{12.4}$ & 56.0 / 60.3$_\impro{4.3}$ \\ 
\midrule
Qwen2-VL (Prompt 1) & 42.0 / 59.0$_\impro{17.0}$ & 55.9 / 61.4$_\impro{5.5}$ \\
Qwen2-VL (Prompt 2) & 46.0 / 57.6$_\impro{11.6}$ & 57.2 / 60.6$_\impro{3.4}$ \\
Qwen2-VL (Prompt 3) & 41.9 / 54.9$_\impro{13.0}$ & 56.9 / 60.9$_\impro{4.0}$ \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table}


==> tables/iter_more.tex <==
\begin{table*}[t] 
\small
\begin{center}
\caption{Performance of different refinement steps.}
\label{tab:iter_more}
\begin{tabular}{l|cccccccccc}
\toprule[1.5pt]
Steps & 1 & 2 & 3 & 4& 5& 6& 7& 8& 9& 10  \\ 
\midrule
Capsbench Acc. & 43.18&	53.39&	56.86&	57.59	&57.65	&58.45&	58.23&	58.73&	57.99	&58.62
  \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table*}


==> tables/iterative.tex <==
% \begin{table*}[]
% \small
% \tabcolsep=0.15cm
% \caption{Performance of \modelname and \modeldpo under different initial MLLM recaptioning models. In CapsBench, Acc. denotes overall accuracy, and Rel.Pos. indicates relative position accuracy. In CompreCap, Obj., Pix., Attr., and Rel. represent object coverage, pixel coverage, attribute score, and relation score, respectively. Green text indicates improvement. \modelname shows significant improvements over the original captions, while \modeldpo achieves performance comparable to that of \modelname.
% }
% \label{tab:iter}
% \begin{tabular}{l|ccc|cccc|c}
% \toprule[1.5pt]
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{CapsBench}    & \multicolumn{4}{c|}{CompreCap}     &  \multicolumn{1}{c}{Amber}    \\ \cmidrule{2-9}

%      & Acc. $\uparrow$ & Color $\uparrow$  & Rel. Pos.$\uparrow$ & Obj.$\uparrow$    & Pix.$\uparrow$   & Attr.$\uparrow$    & Rel.$\uparrow$ & Over. $\uparrow$  \\ \midrule
     
% Qwen2-VL Init.    & 42.02     & 48.11  & 32.41  & 69.82  & 60.02  & 2.66 & 2.81  & 59.7       \\ 
% + \modeldpo   
% & 55.32$_\impro{12.30}$ & 66.67$_\impro{18.56}$ & 55.09$_\impro{22.68}$  &  74.80$_\impro{4.98}$   & \textbf{63.35}$_\impro{3.33}$ & 2.84$_\impro{0.18}$ & \textbf{2.84}$_\impro{0.03}$ &  60.6  \\ 

% % & 53.28$_\impro{11.26}$ & 68.38$_\impro{20.27}$ & 50.00$_\impro{17.59}$  & 74.41$_\impro{4.9}$   & 63.45$_\impro{3.43}$ & 2.84$_\impro{0.18}$ & 2.83$_\impro{0.02}$ & 25.8$_\impro{-}$ & 25.8$_\impro{-}$\\ 
% + \modelname($N=2$)         & \textbf{59.02}$_\impro{17.00}$ & \textbf{67.14}$_\impro{19.03}$ & \textbf{59.51}$_\impro{27.10}$  & \textbf{75.04}$_\impro{5.22}$ & 63.04$_\impro{3.02}$ & \textbf{2.85}$_\impro{0.19}$ & 2.82$_\impro{0.01}$ & 62.2  \\ \midrule

% % CogVLM Init.        & 45.1 & 47.77 & 39.81 & 68.54 & 59.21 & 2.57 & 2.61 &\update{48.7} & \update{4.4}\\ 
% % \modeldpo     & & & & & & &  \\ 
% % \modelname$(N=2)$          & 57.51$_\impro{12.41}$ & 63.67$_\impro{---}$ & 48.76$_\impro{---}$ & 75.37$_\impro{6.83}$ & 61.65$_\impro{2.44}$ & 2.78$_\impro{0.21}$ & 2.75$_\impro{0.14}$ & \update{27.1} & \update{2.9}
% % \\
% LLaVA-1.5 Init.        & 29.51 & 27.84 & 18.06 & 57.14 & 44.48 & 2.02 & 2.38 & 44.7\\ 
% + \modeldpo     & 46.16 & 49.61 & 38.70 & 66.68 &56.52 & 2.53 &  2.43 & 53.1\\ 
% + \modelname$(N=2)$          & 53.13$_\impro{23.62}$ & 61.07$_\impro{33.23}$ & 48.10$_\impro{30.04}$ & 76.38 & 61.49 & 2.82 & 2.82 & 59.7\\
% \bottomrule[1.5pt]
% \end{tabular}
% \end{table*}


\begin{table*}[]
\small
\tabcolsep=0.17cm
\caption{Performance of \modelname and \modeldpo under different initial MLLM recaptioning models. For \modeldpo, we use the corresponding MLLM as the base model. In CapsBench, \textit{Acc.} denotes overall accuracy, and \textit{Rel.Pos.} indicates relative position accuracy. In CompreCap, \textit{Obj.}, \textit{Pix.}, \textit{Attr.}, and \textit{Rel.} represent object coverage, pixel coverage, attribute score, and relation score, respectively. \textit{Over.} in Amber refers to overall performance (see \textsection~\ref{sec:app_bench} for details). Green text indicates improvements. \modelname demonstrates significant gains over the original captions, while \modeldpo achieves performance close to that of \modelname.
}
\label{tab:iter}
\begin{tabular}{l|lll|l|llll}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{CapsBench} & Amber & \multicolumn{4}{c}{CompreCap}  \\ \cmidrule{2-9}
     & Acc. $\uparrow$ & Color $\uparrow$ & Rel. Pos. $\uparrow$ & Over. $\uparrow$ & Obj. $\uparrow$ & Pix. $\uparrow$ & Attr. $\uparrow$ & Rel. $\uparrow$ \\ \midrule

Qwen2-VL Init. & 42.0 & 48.1 & 32.4 & 59.7 & 69.82 & 60.02 & 2.66 & 2.81 \\
+ \modeldpo 
& 55.3$_\impro{13.3}$ & 66.7$_\impro{18.6}$ & 55.1$_\impro{22.7}$ & 60.6$_\impro{0.9}$ & 74.80$_\impro{4.98}$ & \textbf{63.35}$_\impro{3.33}$ & 2.84$_\impro{0.18}$ & \textbf{2.84}$_\impro{0.03}$ \\
+ \modelname($N=2$) 
& \textbf{59.0}$_\impro{17.0}$ & \textbf{67.1}$_\impro{19.0}$ & \textbf{59.5}$_\impro{27.1}$ & \textbf{62.2}$_\impro{2.5}$ & \textbf{75.04}$_\impro{5.22}$ & 63.04$_\impro{3.02}$ & \textbf{2.85}$_\impro{0.19}$ & 2.82$_\impro{0.01}$ \\ \midrule

LLaVA-1.5 Init. & 29.5 & 27.8 & 18.1 & 44.7 & 57.14 & 44.48 & 2.02 & 2.38 \\
+ \modeldpo 
& 46.2$_\impro{16.7}$ & 49.6$_\impro{21.8}$ & 38.7$_\impro{20.6}$ & 53.1$_\impro{8.4}$ &  66.68$_\impro{9.54}$ & 56.52$_\impro{12.04}$ & 2.53$_\impro{0.51}$ & 2.43$_\impro{0.05}$ \\
+ \modelname($N=2$) 
& \textbf{53.1}$_\impro{23.6}$ & \textbf{61.1}$_\impro{33.3}$ & \textbf{48.1}$_\impro{30.0}$ & \textbf{59.7}$_\impro{15.0}$ & \textbf{76.38}$_\impro{19.24}$ & \textbf{61.49}$_\impro{17.01}$ & \textbf{2.82}$_\impro{0.80}$ & \textbf{2.82}$_\impro{0.44}$ \\
\bottomrule[1.5pt]
\end{tabular}
\end{table*}


==> tables/model_abl.tex <==
\begin{table}[t] 
\small
\begin{center}
\tabcolsep=0.15cm
\caption{Ablation studies. 
}
\vspace{-1mm}
	\label{tab:model_abl}
		 \begin{tabular}{l|cccc}
		\toprule[1.5pt]
		 \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{CapsBench}   \\  
         \cmidrule{2-5}
        & Acc. & Color  & Rel. Pos. & Shape\\
        \midrule 
        \modelname & \textbf{59.02}  & \textbf{67.14} & \textbf{59.51} & \textbf{53.68} \\
        \modeldpo  &\underline{55.32} & \underline{66.67} & \underline{55.09} & \underline{50.29}  \\
                \midrule
  (a) wo/ tips & 54.33 & 62.23 & 50.95 & 42.11\\
        (b) wo/ output analy. &50.40 & 62.54 & 53.24 & 36.36\\
        (c) finetune w/ pos.& 51.16 & 59.79 & 51.85 & 32.32\\
        (d) infer with ICL & 45.26 &49.83 &42.13 &26.26  \\


                 
   
		\bottomrule[1.5pt]
	\end{tabular}

\end{center}

\end{table}

==> tables/prompt.tex <==
% \begin{table*}[]
% \caption{Detailed performance of \modelname across different initial prompts.}
% \label{tab:app_prompt}
% \begin{tabular}{l|cccc|cccc}
% \toprule[1.5pt]
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{CapsBench}    & \multicolumn{4}{c}{CompreCap}    \\ \cmidrule{2-9}

%      & Acc. & Color & Shape & Rel. Pos. & Obj.    & Pix.   & Rel.    & Attr.   \\ \midrule
     
% Prompt \#1 & 42.02 & 48.11 & 27.27 & 32.41& 69.82  & 60.02  & 2.66 & 2.81\\
% + \modelname & 59.02 & 67.14 & 53.68 & 59.51& 75.04$_\impro{5.22}$ & 63.04$_\impro{3.02}$ & 2.85$_\impro{0.19}$ & 2.82$_\impro{0.01}$\\ \midrule
% Prompt \#2 & 45.97 & 49.14 & 23.22 & 40.74 &69.29 & 60.41 & 2.69 & 2.62\\
% + \modelname & 57.64& 65.45 & 39.08 & 56.45 & 74.83 & 62.65 & 2.80 & 2.79\\
% \midrule
% Prompt \#3 & 41.85 & 43.30 & 23.23 & 36.11 & 68.46 & 58.89 & 2.72 & 2.59\\
% + \modelname &54.85 &66.54 & 47.25 & 52.85 & 75.15 & 62.40 & 2.80 & 2.82\\
% \bottomrule[1.5pt]
% \end{tabular}
% \end{table*}
\begin{table*}[]
\caption{Detailed performance of \modelname across different initial prompts.}
\small
\tabcolsep=0.18cm
\label{tab:app_prompt}
\begin{tabular}{l|llll|llll}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{CapsBench}    & \multicolumn{4}{c}{CompreCap}    \\ \cmidrule{2-9}
     & Acc. & Color & Shape & Rel. Pos. & Obj.    & Pix.   & Rel.    & Attr.   \\ \midrule[1pt]
     
Prompt \#1 & 42.02 & 48.11 & 27.27 & 32.41 & 69.82  & 60.02  & 2.66 & 2.81\\
+ \modelname & 59.02$_\impro{17.00}$ & 67.14$_\impro{19.03}$ & 53.68$_\impro{26.41}$ & 59.51$_\impro{27.10}$ & 75.04$_\impro{5.22}$ & 63.04$_\impro{3.02}$ & 2.85$_\impro{0.19}$ & 2.82$_\impro{0.01}$\\ \midrule

Prompt \#2 & 45.97 & 49.14 & 23.22 & 40.74 & 69.29 & 60.41 & 2.69 & 2.62\\
+ \modelname & 57.64$_\impro{11.67}$ & 65.45$_\impro{16.31}$ & 39.08$_\impro{15.86}$ & 56.45$_\impro{15.71}$ & 74.83$_\impro{5.54}$ & 62.65$_\impro{2.24}$ & 2.80$_\impro{0.11}$ & 2.79$_\impro{0.17}$\\ \midrule

Prompt \#3 & 41.85 & 43.30 & 23.23 & 36.11 & 68.46 & 58.89 & 2.72 & 2.59\\
+ \modelname & 54.85$_\impro{13.00}$ & 66.54$_\impro{23.24}$ & 47.25$_\impro{24.02}$ & 52.85$_\impro{16.74}$ & 75.15$_\impro{6.69}$ & 62.40$_\impro{3.51}$ & 2.80$_\impro{0.08}$ & 2.82$_\impro{0.23}$\\

\bottomrule[1.5pt]
\end{tabular}
\end{table*}


==> tables/prompt_template.tex <==
% \begin{table*}[ht!]


% \begin{tcolorbox}[breakable]

% {\normalsize \textbf{================  ~\textsc{Prompt in the Refinement Procedure}~ ================}}

% \tcblower

% We are working on a project that involves generating captions for images and using these captions to reconstruct the images. The process follows these steps:

% \begin{enumerate}
%     \item \textbf{Original Image (First Image):} A caption is generated based on this image.
%     \item \textbf{Reconstructed Image (Second Image):} The generated caption is used as input for a text-to-image model to create this image.
% \end{enumerate}

% \textbf{Your Task}

% Compare the \textbf{original} and \textbf{reconstructed} images, analyzing their differences to identify potential improvements for the original caption. Based on your observations, provide a \textbf{revised caption} that could enhance the reconstruction quality.
% ~\\

% \textbf{Guidelines for Comparison}

% When analyzing the differences between the two images, consider the following aspects:

% \begin{itemize}
%     \item \textbf{Visual Details:} Color, shape, texture, and material of objects.
%     \item \textbf{Composition \& Layout:} Object positioning, spatial relationships, and overall scene structure.
%     \item \textbf{Human Attributes (if applicable):} Pose, facial expression, skin tone, clothing, and hairstyle.
%     \item \textbf{Perspective \& Style:} Type of image, camera angle, depth of field, lighting, and artistic style.
%     \item \textbf{Text in the Image:} Accuracy of any visible words, symbols, or signs.
%     \item \textbf{Image Quality:} Blurriness, artifacts, or inconsistencies in object rendering.
%     \item \textbf{World Knowledge:} Proper nouns or specific real-world references that should be preserved.
%     \item \textbf{Color Aesthetics:} Color palette, grading, and overall mood consistency.
% \end{itemize}

% \textbf{How to Improve the Caption}
% \begin{itemize}
%     \item \textbf{Add missing details} that were lost in reconstruction.
%     \item \textbf{Clarify ambiguous descriptions} to provide more precise information.
%     \item \textbf{Correct any inaccuracies} based on observed differences.
%     \item \textbf{Specify key attributes} (e.g., ``a red leather couch'' instead of ``a couch'').
% \end{itemize}

% Your revised caption should aim to \textbf{reduce discrepancies} between the original and reconstructed images while maintaining a natural and informative description. You are encouraged to make the revised caption less than 512 tokens.

% ~\\
% Now I provide the original image, reconstructed image, and the original caption: \texttt{\{orig\_caption\}}.

% ~\\
% Please give me the revised caption that you believe could enhance the reconstruction quality (i.e., make the new reconstructed image more like the original one at pixel level), enclosed with \texttt{<revised caption>}. And provide your analysis enclosed with \texttt{<analysis>} after.




% \end{tcolorbox}
% \caption{The prompt used to query GPT-4o in the refinement procedure.}
% \label{tab:gpt4_prompt}
% \end{table*}


\begin{table*}[ht!]
\begin{tcolorbox}[breakable]

{\normalsize \textbf{================  ~\textsc{Prompt in the Refinement Procedure}~ ================}}

\tcblower

We are working on a project that involves generating captions for images and using these captions to reconstruct the images. The process follows these steps:

\hangindent=2em\hangafter=1
\textbf{1. Original Image (First Image):} A caption is generated based on this image.

\hangindent=2em\hangafter=1
\textbf{2. Reconstructed Image (Second Image):} The generated caption is used as input for a text-to-image model to create this image.

\bigskip

\textbf{Your Task}

Compare the \textbf{original} and \textbf{reconstructed} images, analyzing their differences to identify potential improvements for the original caption. Based on your observations, provide a \textbf{revised caption} that could enhance the reconstruction quality.

\bigskip

\textbf{Guidelines for Comparison}

\hangindent=2em\hangafter=1
\textbf{• Visual Details:} Color, shape, texture, and material of objects.

\hangindent=2em\hangafter=1
\textbf{• Composition \& Layout:} Object positioning, spatial relationships, and overall scene structure.

\hangindent=2em\hangafter=1
\textbf{• Human Attributes (if applicable):} Pose, facial expression, skin tone, clothing, and hairstyle.

\hangindent=2em\hangafter=1
\textbf{• Perspective \& Style:} Type of image, camera angle, depth of field, lighting, and artistic style.

\hangindent=2em\hangafter=1
\textbf{• Text in the Image:} Accuracy of any visible words, symbols, or signs.

\hangindent=2em\hangafter=1
\textbf{• Image Quality:} Blurriness, artifacts, or inconsistencies in object rendering.

\hangindent=2em\hangafter=1
\textbf{• World Knowledge:} Proper nouns or specific real-world references that should be preserved.

\hangindent=2em\hangafter=1
\textbf{• Color Aesthetics:} Color palette, grading, and overall mood consistency.

\bigskip

\textbf{How to Improve the Caption}

\hangindent=2em\hangafter=1
\textbf{• Add missing details} that were lost in reconstruction.

\hangindent=2em\hangafter=1
\textbf{• Clarify ambiguous descriptions} to provide more precise information.

\hangindent=2em\hangafter=1
\textbf{• Correct any inaccuracies} based on observed differences.

\hangindent=2em\hangafter=1
\textbf{• Specify key attributes} (e.g., “a red leather couch” instead of “a couch”).

\bigskip

Your revised caption should aim to \textbf{reduce discrepancies} between the original and reconstructed images while maintaining a natural and informative description. You are encouraged to make the revised caption less than 512 tokens.

\bigskip

Now I provide the original image, reconstructed image, and the original caption: \texttt{\{orig\_caption\}}.

\bigskip

Please give me the revised caption that you believe could enhance the reconstruction quality (i.e., make the new reconstructed image more like the original one at pixel level), enclosed with \texttt{<revised caption>}. And provide your analysis enclosed with \texttt{<analysis>} after.

\end{tcolorbox}
\caption{The prompt used to query GPT-4o in the refinement procedure.}
\label{tab:gpt4_prompt}
\end{table*}


==> tables/reviser.tex <==
\begin{table}[t] 
\small
\begin{center}
\caption{Performance of different refinement models. For CapsBench, we report overall accuracy.}
\label{tab:refine}
\begin{tabular}{l|c}
\toprule[1.5pt]
Model & CapsBench  \\ 
\midrule
Qwen2-VL as reviser & 42.0 / 45.8$_\impro{3.8}$ \\
GPT-4o as reviser & 42.0 / 59.0$_\impro{17.0}$  \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table}


==> tables/rpos_res.tex <==
\begin{table*}[ht!]
\caption{An example of an original caption and its refined version.
}

\begin{tcolorbox}

% {\normalsize \textbf{============  ~\textsc{Different prompts to generate initial captions}~ ============}}

% \tcblower


\textbf{Original:}

The image depicts a scene from an animated series, featuring three characters seated on a green, ornate couch. The man has red hair and is dressed in a brown suit with a white shirt and tie. The woman has blonde hair styled in a high ponytail and is wearing a blue dress with a white collar. The child has pink hair and is dressed in a red outfit with a green bow. The background is a simple, muted color, focusing attention on the characters. The overall style is vibrant and detailed, typical of anime art. 

~\\
\textbf{Revised:}

The image depicts a scene from an animated series featuring three characters seated on a green, ornate couch with an elaborate, dark wooden backrest. The man <*\textbf{on the left}*> has light pink hair styled in a straight cut and is dressed in a brown suit with a white shirt and a black tie. The woman <*\textbf{on the right}*> has long blonde hair styled in a sleek, high ponytail and is wearing a light blue dress with a white collar and a sash tied at the waist. The child <*\textbf{in the center}*> has light pink hair in a cute bob cut and is dressed in a red outfit with a bright green bow. The background is plain with subtle tones, highlighting the characters. The overall style is soft and detailed, typical of high-quality anime art, with pastel colors. <*\textbf{The composition is a medium shot, allowing clear visibility of the characters' attire and expressions.}*>



\end{tcolorbox}

\label{tab:rel}
\end{table*}

==> tables/t2i.tex <==
\begin{table}[t] 
\vspace{-0mm}
\begin{center}
\small
\tabcolsep=0.10cm
\caption{Evaluation of a text-to-image generation model trained with original captions versus captions refined by our \modeldpo model. \textit{Rel.} and \textit{Attr.} represent relation and attribute respectively.
}
	\label{tab: t2i}
	\begin{tabular}{l|ccc|c}
		\toprule[1.5pt]
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{DPG-Bench}  &  \multirow{2}{*}{VQAScore}  \\   
         & Rel. & Attr. & Overall & \\
        \midrule

        FLUX w/ Init. Cap. 	& 89.95 &	80.08 & 78.50 & 0.84\\
        FLUX w/ \modeldpo 	& \textbf{90.55} &	\textbf{82.83}	& 	\textbf{80.34} & \textbf{0.85}\\

                 
   
		\bottomrule[1.5pt]
	\end{tabular}
\end{center}

\end{table}

==> tables/t2i_ext.tex <==
\begin{table*}[t] 
\vspace{-0mm}
\label{tab:app_t2i}
\begin{center}
\small
% \tabcolsep=0.2cm
\caption{Extended version of the evaluation of the text-to-image model.
}
	\label{tab:t2i_exp}
	\begin{tabular}{l|ccccc|c}
		\toprule[1.5pt]
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{DPG-Bench}  &  \multirow{2}{*}{VQAScore}  \\   
        \cmidrule{2-6} 
        & Entity & Relation & Attribute & Global & Overall & \\
        \midrule

        FLUX w/ Init. Cap. & 85.110	& 89.950 &	80.080 &72.414 & 78.502 & 0.841\\
        FLUX w/ \modelname-DPO & \textbf{86.850}	& \textbf{90.551} &	\textbf{82.831}	&\textbf{75.172} & 	\textbf{80.336} & \textbf{0.852}\\

                 
   
		\bottomrule[1.5pt]
	\end{tabular}
\end{center}

\end{table*}

==> tables/time.tex <==
\begin{table}[t] 
\small
\begin{center}
\caption{Inference time comparison of different models. "RICO wo/ ana." denotes the RICO model without the necessity to generate an analysis process. }
\label{tab:app_time}
\begin{tabular}{l|c}
\toprule[1.5pt]
Model & Time (s)  \\ 
\midrule
RICO & 40.1 \\
RICO wo/ ana. & 37.8  \\
RICO-Flash & 4.2 \\
\bottomrule[1.5pt]
\end{tabular}
\end{center}
\end{table}

